Some challenges of diffused interfaces in implicit-solvent models

The standard Poisson-Boltzmann model for molecular electrostatics assumes a sharp variation of the permittivity and salt concentration along the solute-solvent interface. The discontinuous field parameters are not only difficult numerically, but also are not a realistic physical picture, as it forces the dielectric constant and ionic strength of bulk in the near-solute region. An alternative to alleviate some of these issues is to represent the molecular surface as a diffuse interface, however, this also presents challenges. In this work we analysed the impact of the shape of the interfacial variation of the field parameters in solvation and binding energy. However we used a hyperbolic tangent function ($\tanh(k_p x)$) to couple the internal and external regions, our analysis is valid for other definitions. Our methodology was based on a coupled finite element (FEM) and boundary element (BEM) scheme that allowed us to have a special treatment of the permittivity and ionic strength in a bounded FEM region near the interface, while maintaining BEM elsewhere. Our results suggest that the shape of the function (represented by $k_p$) has a large impact on solvation and binding energy. We saw that high values of $k_p$ induce a high gradient on the interface, to the limit of recovering the sharp jump when $k_p\to\infty$, presenting a numerical challenge where careful meshing is key. Using the FreeSolv database to compare with molecular dynamics, our calculations indicate that an optimal value of $k_p$ for solvation energies was around 3. However, more challenging binding free energy tests make this conclusion more difficult, as binding showed to be very sensitive to small variations of $k_p$. In that case, optimal values of $k_p$ ranged from 2 to 20.

==> Exhibit.tex <==

\begin{table}[h]
\caption{Breakdown Binding Energy into Solvation and Coulomb Energy (in [kcal/mol]) in BEM-FEM-BEM Hyperbolic Tangent for different structures.}
\begin{tabular*}{\tblwidth}{@{}LL@{}LL@{}LL@{}LL@{}LL@{}}
\toprule
Name & kp & Structure & Solvation & Coulomb  & Binding \\ % Table header row
\midrule
1BBZ & 6 & Protein & -224.730 & -7142.558  & -2.696 \\
     &   & Ligand & -49.094 & -799.628   & \\
     &   & Complex & -267.514  & -7951.191 &   \\
\cline{2-6}
     & 14 & Protein & -156.069 & -7142.558  &  -8.746  \\
     &   & Ligand & -35.085 & -799.628   & \\
     &   & Complex & -190.895  & -7951.191 &   \\
\cline{2-6}
     & 11.50 & Protein & -164.530 & -7142.558  & -7.977 \\
     &   & Ligand & -36.858 & -799.628   & \\
     &   & Complex & -200.359  & -7951.191 &   \\
\toprule
1SE0 & 6 & Protein & -519.545 & -13811.001  & -32.349 \\
     &   & Ligand & -56.328 & -562.455   & \\
     &   & Complex & -490.117  & -14491.560 &   \\
\cline{2-6}
     & 14 & Protein & -382.717 & -7142.558  & -49.150  \\
     &   & Ligand & -41.322 & -799.628   & \\
     &   & Complex & -355.084  & -7951.191 &   \\
\cline{2-6}
     & 2.47  & Protein & -727.545 & -7142.558  & -9.500  \\
     &   & Ligand & -76.646 & -799.628   & \\
     &   & Complex & -695.587  & -7951.191 &   \\
\toprule
1BRS & 6 & Protein 1 & -344.175 & -16874.665 & -53.548 \\
     &   & Protein 2 & -462.959	& -13333.959 & \\
     &   & Complex   &	-567.175 & -30502.132 & \\
\cline{2-6}
     & 14 & Protein 1  & -232.483 & -16874.665 & -91.313 &  \\
     &   & Protein 2 &	-350.604 & -13333.959  & \\
     &   & Complex  & -380.893 & -30502.132  & \\
\cline{2-6}
    & 2.17 & Protein 1 & -542.164 & -16874.665 & 0.919 &  \\
     &   & Protein 2 & -645.992	& -13333.959  & \\
     &   & Complex  &  -893.729	& -30502.132  & \\
\toprule
1EMV & 6 & Protein 1 & -705.110 & -11926.994 & -20.376  \\
     &   & Protein 2 & -694.009 & -19973.586 & \\
     &   & Complex   &	-892.855 & -32427.219 & \\
\cline{2-6}
     & 14 & Protein 1 & -581.451 & -11926.994 & -53.154  \\
     &   & Protein 2 & -496.085 & -19973.586 & \\
     &   & Complex   &	-604.052 & -32427.219 & \\
\cline{2-6}
     & 3.97 & Protein 1 & -810.525 & -11926.994 & 2.228  \\
     &   & Protein 2 & -871.377 & -19973.586 & \\
     &   & Complex   & -1153.035 & -32427.219 & \\
\toprule
1JTG & 6 & Protein 1 & -795.481 & -40563.513 & -9.832  \\
     &   & Protein 2 & -407.975 & -22906.586 & \\
     &   & Complex   &	-1093.447 & -63589.939 & \\
\cline{2-6}
     & 14 & Protein 1 & -564.168 & -40563.513 & -61.147  \\
     &   & Protein 2 & -272.488 & -22906.586 & \\
     &   & Complex  &	-777.962 & -63589.939 & \\
\cline{2-6}
     & 5.37 & Protein 1 & -851.523 & -40563.513 & 0.417   \\
     &   & Protein 2 & -441.929 & -22906.586 & \\
     &   & Complex   &	-1173.194 & -63589.939 & \\
\bottomrule
\label{table:7Proteinas_Desglose}
\end{tabular*}
\end{table}

\begin{table}[h]
\caption{Continuation of breakdown Binding Energy into Solvation and Coulomb Energy (in [kcal/mol]) in BEM-FEM-BEM Hyperbolic Tangent for different structures.}
\begin{tabular*}{\tblwidth}{@{}LL@{}LL@{}LL@{}LL@{}LL@{}}
\toprule
Name & kp & Structure & Solvation & Coulomb  & Binding \\ % Table header row
\midrule
1BEB & 6 & Protein 1 & -1030.465 & -22537.376 & 21.274  \\
     &   & Protein 2 & -997.504 & -22661.424 & \\
     &   & Complex   & -2378.778 & -44826.716 & \\
\cline{2-6}
     & 14 & Protein 1 & -822.205 & -22537.376 & 0.713   \\
     &   & Protein 2 & -803.149 & -22661.424 & \\
     &   & Complex   & -1996.724 & -44826.716 & \\
\cline{2-6}
     & 17.55  & Protein 1 & -801.101 & -22537.376 & -1.626 \\
     &   & Protein 2 & -783.685 & -22661.424 & \\
     &   & Complex   & -1958.495 & -44826.716 & \\
\toprule
1A3N & 6 & Protein 1 & -993.352 & -38235.611 & 61.904  \\
     &   & Protein 2 & -860.966 & -38451.168 & \\
     &   & Complex   & -1662.440 & -76816.753 & \\
\cline{2-6}
     & 14 & Protein 1 & -738.082 & -38235.611 & -19.493 \\
     &   & Protein 2 & -610.340 & -38451.168 & \\
     &   & Complex   & -1237.941 & -76816.753 & \\
\cline{2-6}
     & 10.57 & Protein 1 & -786.141 & -38235.611 & 0.155   \\
     &   & Protein 2 & -657.438 & -38451.168 & \\
     &   & Complex   & -1313.451 & -76816.753 & \\
\bottomrule
\label{table:7Proteinas_Desglose}
\end{tabular*}
\end{table}

\subsection{Optimizacion de la funcion distancia.}
\color{blue}
Para calcular el parametro alfa $\alpha_{i}$ definimos la funcion de distancia entre el vertice $x_{i}$ y la ecuacion lineal $X(\alpha_{i} )$:
\begin{align*} 
    d(\alpha_{i},x_{i})=\left \| X(\alpha_{i} )-x_{i} \right \| = \left \| \left ( X_{a}-x_{i} \right )+\alpha_{i} \left (X_{b}-X_{a}\right ) \right \|
\end{align*}
El $\alpha_{i}$ optimo corresponde a la distancia mas pequeña entre el vertice $x_{i}$ y la ecuacion lineal $X(\alpha_{i} )$, donde se sabe que esta ubicado en el valor entre 0 y 1. Para ello, debemos optimizar la funcion distancia $d(\alpha_{i},x_{i})$ para calcular el alfa optimo, primero necesitamos calcular su primera derivada en funcion de alfa, en su forma espacial:
\begin{align*}
    d(\alpha_{i},x_{i})=\sqrt{\left (x_{1}+\alpha_{i}x_{2}\right)^2+\left (y_{1}+\alpha_{i}y_{2}\right)^2+\left (z_{1}+\alpha_{i}z_{2}\right)^2}
\end{align*}
Donde los parametro adicionales para simplificar la ecuacion corresponden a:
\begin{multline}
\left ( X_{a}-x_{i} \right ) =\left (\left (x_{a}-\bar{x}_{i} \right ), \left (y_{a}-\bar{y}_{i} \right ) ,\left (z_{a}-\bar{z}_{i} \right ) \right ) \\
=\left (x_{1},y_{1},z_{1}  \right ) \\
\left (X_{b}-X_{a} \right ) =\left (\left (x_{b}-x_{a} \right ), \left (y_{b}-y_{a} \right ) ,\left (z_{b}-z_{a} \right ) \right ) \\
 =\left (x_{2},y_{2},z_{2}  \right ) \\
\end{multline}
Se deriva la funcion de la distancia:
\begin{align*} 
    \frac{\partial d(\alpha)}{\partial \alpha }=\frac{2x_{2}\left (x_{1}+\alpha_{i}x_{2} \right )+2y_{2}\left (y_{1}+\alpha_{i}y_{2} \right )+2z_{2}\left (z_{1}+\alpha_{i}z_{2} \right )}{2\sqrt{\left (x_{1}+\alpha_{i}x_{2}\right)^2+\left (y_{1}+\alpha_{i}y_{2}\right)^2+\left (z_{1}+\alpha_{i}z_{2}\right)^2 }}
\end{align*}
Se reodenar algebraicamente la primera derivada:
\begin{align*} 
    \frac{\partial d(\alpha)}{\partial \alpha }=\frac{\alpha_{i}\left (x_{2}^{2}+y_{2}^{2} +z_{2}^{2}  \right )+x_{1}x_{2}+y_{1}y_{2}+z_{1}z_{2}}{\sqrt{\left (x_{1}+\alpha_{i}x_{2}^2\right )^2+\left (y_{1}+\alpha_{i}y_{2}^2\right )^2+\left (z_{1}+\alpha_{i}z_{2}^2\right )^2 }}
\end{align*}
Finalmente, al escribir el resultado en su forma vectorial en vez de forma espacial, la primera derivada de la distancia corresponde a:
\begin{align*} 
    \frac{\partial d(\alpha_{i} ,x_{i})}{\partial \alpha }=\frac{\alpha_{i}\left \| X_{b}-X_{a} \right \|^{2}+\left (X_{a}-x_{i}\right )\cdot \left (X_{b}-X_{a}\right )}{\left \| \left (X_{a}-x_{i}\right )+\alpha_{i} \left (X_{b}-X_{a}\right ) \right \|}
\end{align*}

Para encontrar el valor optimo de alfa, la primera derivada de la distancia se iguala a 0, que corresponde a la ubicacion del valor minimo de la funcion distancia, encontrando el valor optimo alfa que necesitamos:
\begin{align*} 
    \frac{\partial d(\alpha ,x)}{\partial \alpha }=0 
\end{align*}
\begin{align*} 
    \frac{\alpha_{i}\left \| X_{b}-X_{a} \right \|^{2}+\left (X_{a}-x_{i}\right )\cdot \left (X_{b}-X_{a}\right )}{\left \| \left (X_{a}-x_{i}\right )+\alpha_{i} \left (X_{b}-X_{a}\right ) \right \|}=0
\end{align*}
Debido a que necesitamos la distancia mas pequeña, y no la distancia sea exactamente igual a 0, por el motivo que al generar la malla volumetrica, es dificil el vertice $x_{i}$ coincida exactamente  $X(\alpha_{i} )$, el denominador de la funcion se considera no nulo: 
\begin{align*} 
    \alpha_{i}\left \| X_{b}-X_{a} \right \|^{2}+\left (X_{a}-x_{i}\right )\cdot \left (X_{b}-X_{a}\right )=0
\end{align*}

Despejando algebraicamente, el alfa optimo es:
\begin{align*} 
    \alpha_{i}(x_{i})=-\frac{(X_{a}-x_{i})\cdot (X_{b}-X_{a})}{\left \| X_{b}-X_{a} \right \|^{2}}
\end{align*}
\color{black}

% \subsection{Gaussian Convolution Surface.}
% \color{cyan}
% \begin{align*}
% H(x)=\left\{\begin{matrix}
% 1 & x \leq 0\\ 
% 0 & x > 0
% \end{matrix}\right. \quad  K(x)=\frac{e^{-\frac{x^{2}}{2 \sigma^{2}}}}{\sigma \sqrt{2 \pi}}
% \end{align*}

% \begin{align*}
% \begin{matrix}
%     (H*K)(x)=\int_{-\infty}^{\infty}H(x-t)K(t)dt \\ 
%     (H*K)(x)=\int_{-\infty}^{\infty}H(t)K(x-t)dt=\int_{-\infty}^{0}K(x-t)dt \\ 
%     (H*K)(x)=\int_{-\infty}^{0}\frac{e^{-\frac{(x-t)^{2}}{2 \sigma^{2}}}}{\sigma \sqrt{2 \pi}}dt =\frac{1}{2}-\frac{1}{2}erf\left ( \frac{x}{\sigma\sqrt{2}} \right ) \\ 
% \end{matrix}
% \end{align*}

% \begin{align*}
% S(\alpha,\sigma) = (H*K)(\alpha)=\frac{1}{2}-\frac{1}{2}erf\left ( \frac{\alpha-0.5}{\sigma\sqrt{2}} \right )
% \end{align*}

\subsection{Tabla adicional.}

Extrapolación de Richardson.
\begin{align*} 
    r= \frac{v_{2}}{v_{1}} \quad p=\frac{log\left ( \left ( \frac{E_{1}-E_{2}}{E_{2}-E_{3}} \right ) \right )}{log\left ( r \right )} \quad E_{R}=E_{2}+\frac{E_{2}-E_{1}}{r^{p}-1} 
\end{align*}

The growthfactor option helps control the transition from small to larger sizes within the mesh. The value specified will be the approximate ratio in the size of adjacent elements going from the boundary into the interior of the mesh. For example, a growthfactor of 1.1 allows approximately 10\% growth in each layer of adjacent elements.
\color{black}
%https://coreform.com/cubit_help/mesh_generation/meshing_schemes/traditional/tetmesh.htm

\begin{table}[h]
\caption{Solvation Energy  (in [kcal/mol]) for BEM-FEM-BEM Hyperbolic Tangent with kp equal to 6, of Sphere of radius 5 \AA~ and a 3 \AA~ layer.}
\begin{tabular*}{\tblwidth}{@{}LL@{}LL@{}LL@{}LL@{}LL@{}}
\toprule
MSMS & \multicolumn{3}{c}{Mesh vertices} & \multicolumn{2}{c}{Energy}\\
Density & Inner & Outer & FEM & Solvation &  Richardson \\
\midrule
1 & 290	& 788 & 1582 & -68.456 &  \\
1.9 & 566 & 1475 & 4137 & -65.383 &  \\
3.8 & 1149 & 2939 & 9231 & -64.606 &  -64.342 \\
7.5 & 2334 & 5899 & 22164 & -64.064 & -62.824 \\
15 &  4591 & 11924 & 50529 & -63.766 & -63.400  \\
\bottomrule
\end{tabular*}
\end{table}

\subsection{Calculos Opcionales.}

\color{red}
Al trabajar con la tangente hiperbolica con kp=0, es equivalente a trababar con el caso constante, donde la funcion S es igual a 0.5. Por lo tanto, se puede establecer un valor de las siguientes variables:
\begin{align*}
    S_0(x,k_{p}=0) = \frac{1}{2} \\
    \epsilon_i(x)=\epsilon_{i(S_0)} = \frac{(\epsilon_m+\epsilon_s)}{2} \\
    \bar{\kappa_{i}}^{2}(x) = \epsilon_{i(S_0)}\kappa_{i(S_0)}^{2} = \frac{\epsilon_{s}\kappa_{s}^{2}}{2}\\
\end{align*}
Donde al despejar ki, este es igual a:
\begin{align*}
    \kappa_{i(S_0)} = \kappa_{s}\sqrt{\frac{\epsilon_{s}}{\epsilon_{s}+\epsilon_{m}}} 
\end{align*}
\color{black}




